The Strengths and Behavioral Quirks of Java Bytecode Decompilers

During compilation from Java source code to bytecode, some information is irreversibly lost. In other words, compilation and decompilation of Java code is not symmetric. Consequently, the decompilation process, which aims at producing source code from bytecode, must establish some strategies to reconstruct the information that has been lost. Modern Java decompilers tend to use distinct strategies to achieve proper decompilation. In this work, we hypothesize that the diverse ways in which bytecode can be decompiled has a direct impact on the quality of the source code produced by decompilers. We study the effectiveness of eight Java decompilers with respect to three quality indicators: syntactic correctness, syntactic distortion and semantic equivalence modulo inputs. This study relies on a benchmark set of 14 real-world open-source software projects to be decompiled (2041 classes in total). Our results show that no single modern decompiler is able to correctly handle the variety of bytecode structures coming from real-world programs. Even the highest ranking decompiler in this study produces syntactically correct output for 84% of classes of our dataset and semantically equivalent code output for 78% of classes.

==> listings/Foo-Fernflower.tex <==
\begin{lstlisting}[style = Java, float, floatplacement=H, caption={Foo decompiled with \fernflower.}, label={lst:foo-fernflower}]
public class Foo {
  public int foo(int i, int j) {
   while(true) {
     try {
      while(i < j) i = j++ / i;
      ~return j;~
     } catch (RuntimeException var4) {
      i = 10;
     }
   }
  }
}
\end{lstlisting}

==> listings/MutableObject-Fernflower.tex <==
\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of differences in MutableObject original and decompiled with \fernflower sources.}, label={lst:mutable-object-fernflower}]
    public static int toIntValue(final char ch) {...}
	
    public static int toIntValue(final Character ch) {
        Validate.isTrue(ch != null, "The character must not be null");
        `return toIntValue(ch.charValue());`
        @return toIntValue(ch);@
    }
\end{lstlisting}

==> listings/bukkit-jadx-1-decompiled.tex <==
\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Exerpt of org/bukkit/Bukkit.java decompiled.}, label={lst:bukkit-decompiled}] 
public final class Bukkit {
    @private static Server server;@
	[...]
    public static void setServer(Server server) {
        if (server != null) {
            throw new UnsupportedOperationException(
            "Cannot redefine singleton Server");
        }
        ~server = server;~
        [...]
    }
\end{lstlisting}

==> old-text.tex <==

We consider this diversity of implementations as a an opportunity to improve the overall decompilation process. To verify our intuition, we develop a framework for characterizing Java decompilers according to the quality of their results. Our approach allows to assess the decompilation quality from four principal perspectives: syntactic correctness, syntactic distortion, bytecode differences and \semi. For evaluation, we rely on a dataset of $14$ mature open-source Java projects. 


Previous work  by Emmerik~\cite{Emmerik2004} reported on the experience gained from applying decompilers to real-world Java applications. Their experiments demonstrated that decompilation is capable of solving real business problems that require reverse engineering tasks. Posterior work of Hamilton and Danicic~\cite{Hamilton2009} focused on measuring the effectiveness of $12$ Java decompilers using a series of test programs manually created for this purpose. We notice that some of the originally tested decompilers have been updated, some are not available now and there are also some new open-source decompilers which are actively maintained.  To the best of our knowledge, no previous work has focused on studying the diversity of existing decompilers' implementations, and how this diversity can be leveraged in order to enhance overall resilience and performance for this task.





==> tables/diff.tex <==
\begin{table}[ht!]
\centering
\caption{Bytecode difference ratios of recompilable and pass test classes for each decompiler}
\footnotesize
\begin{tabular}{lcccc}
			\hline
			\textbf{Decompiler}  & \textbf{Diff $==$ 0} & \textbf{Diff $\neq$ 0} & \textbf{Ratio} & \textbf{Ratio (Int)} \\
			\hline
    		\cfr & 1114 & 599 & 0.65 & 0.84\\
    		\fernflower & 582 & 853 & 0.41 & 0.59 \\
    		\krakatau  &  187 & 537 &  0.26 & 0.43\\
    		\procyon  & 1278 & 579 & 0.69 & 0.91\\
    		\dava & 173 & 589 & 0.23 & 0.38\\
    		\jd & 1142 & 233 & 0.83 & 0.87\\
    		\jode & 596 & 539 & 0.53 & 0.68\\
    		\jadx & 573 & 835 & 0.41 & 0.59\\
            \hline
		\end{tabular}
	\label{tab:bytecode-diff}
\end{table}



==> utils/util.tex <==
\usepackage{soul}
\usepackage{tikz}

\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}

\makeatletter

\newcommand{\defhighlighter}[3][]{%
  \tikzset{every highlighter/.style={color=#2, fill opacity=#3, #1}}%
}

\defhighlighter{yellow}{.5}

\newcommand{\highlight@DoHighlight}{
  \fill [ decoration = {random steps, amplitude=1pt, segment length=15pt}
        , outer sep = -15pt, inner sep = 0pt, decorate
        , every highlighter, this highlighter ]
        ($(begin highlight)+(0,8pt)$) rectangle ($(end highlight)+(0,-3pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \tikzset{this highlighter/.style={#1}}%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}

\makeatother

% Common abbrev. are set as commands to ensure proper spacing after the dot
\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\aka}{a.k.a.\@\xspace}
\newcommand{\Aka}{A.k.a.\@\xspace}
\newcommand{\Ie}{I.e.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\Cf}{Cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\Eg}{E.g.\@\xspace}
\newcommand{\etal}{et al.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\Wrt}{W.r.t.\@\xspace}
\newcommand{\mc}{Maven Central\@\xspace}
\newcommand{\semi}{semantic equivalence modulo inputs\@\xspace}
\newcommand{\latests}{\text{\texttt{LATESTS}\@\xspace}}
\newcommand{\pas}{\text{\texttt{P}\@\xspace}}
\newcommand{\act}{\text{\texttt{A}\@\xspace}}
\newcommand{\latest}{\text{$latest$\@\xspace}}
\newcommand{\notlatests}{\overline{\latests}}%% NOTE, it should be used in Math mode!

% List of considered decompilers
\newcommand{\krakatau}{\textsf{Krakatau}\@\xspace}
\newcommand{\jode}{\textsf{Jode}\@\xspace}
\newcommand{\cfr}{\textsf{CFR}\@\xspace}
\newcommand{\fernflower}{\textsf{Fernflower}\@\xspace}
\newcommand{\procyon}{\textsf{Procyon}\@\xspace}
%\newcommand{\jd}{\textsf{JD-GUI}\@\xspace}
\newcommand{\jd}{\textsf{JD-Core}\@\xspace}
\newcommand{\jadx}{\textsf{JADX}\@\xspace}
\newcommand{\dava}{\textsf{Dava}\@\xspace}
\newcommand{\meta}{\textsf{Multi-DC}\@\xspace}


\newcommand{\javac}{\textit{javac}\@\xspace}
\newcommand{\ecj}{\textit{ecj}\@\xspace}

\newcommand{\mdg}{MDG\@\xspace}
\newcommand{\mdgl}{$\text{MDG}_L$\@\xspace}
\newcommand{\start}{\texttt{START}\@\xspace}
\newcommand{\snapshot}{\texttt{SNAPSHOT}\@\xspace}
\newcommand{\isPassive}{isPsv}
\newcommand{\orderV}{\displaystyle {<}_{v}}
\newcommand{\orderT}{\displaystyle {<}_{t}}
\newcommand{\lib}{\texttt{LIBS}\@\xspace}

% comment commands for co-authors
\newcommand{\nicolas}[1]{\mynote{Nicolas}{#1}}
\newcommand{\cesar}[1]{\mynote{Cesar}{#1}}
\newcommand{\martin}[1]{\mynote{Martin}{#1}}
\newcommand{\benoit}[1]{\mynote{Benoit}{#1}}
% \renewcommand{\todo}[1]{\mynote{todo}{#1}}

\newcommand{\nbartifacts}{$1,487,956$\@\xspace}
\newcommand{\nblibraries}{$73,653$\@\xspace}

